Concurrency-Preserving and Sound Monitoring of Multi-Threaded Component-Based Systems

This paper addresses the monitoring of logic-independent linear-time user-provided properties in multi-threaded component-based systems. We consider intrinsically independent components that can be executed concurrently with a centralized coordination for multiparty interactions. In this context, the problem that arises is that a global state of the system is not available to the monitor. A naive solution to this problem would be to plug in a monitor which would force the system to synchronize in order to obtain the sequence of global states at runtime. Such a solution would defeat the whole purpose of having concurrent components. Instead, we reconstruct on-the-fly the global states by accumulating the partial states traversed by the system at runtime. We define transformations of components that preserve their semantics and concurrency and, at the same time, allow to monitor global-state properties. Moreover, we present RVMT-BIP, a prototype tool implementing the transformations for monitoring multi-threaded systems described in the BIP (Behavior, Interaction, Priority) framework, an expressive framework for the formal construction of heterogeneous systems. Our experiments on several multi-threaded BIP systems show that RVMT-BIP induces a cheap runtime overhead.

==> RV_of_CBS.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Runtime Monitoring of Component-Based Systems}
\label{sect-RV}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
From the results of the previous work~\cite{FalconeJNBB15} we are able to monitor a CBS with global state semantics when global states of the system is always available during the system's run. 
This monitor takes the input in form of trace in global states semantics and produces a verdict on the sequence of global states read so far.
Such monitor are independent from any specification formalism used to generate them and are able to check any specification expressing a linear temporal specification.  
%\subsection{Specification for component-based systems}
%\subsection{Verification monitor}
%\subsection{Trace of component-based systems}

==> motivating_example.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%
\section{Motivating Example}
%%%%%%%%%%%%%%%%%%%%%%%
%
Let us consider an example in which we can illustrate the problem intuitively.
%
%\begin{example}[Component-based system]
%\label{example-motivating}
Figure~\ref{fig:example} shows a component-based system consist of four components \textit{Task generator}, \textit{Worker1}, \textit{Worker2},  \textit{Worker3} with initial state  \textit{ready}, \textit{free}, \textit{free}, \textit{free} respectively and glue which defines how components interact together consist of ten interactions $\gamma=\{E_{12}, E_{13}, E_{23}, M_1, M_2, M_3, F_1, F_2, F_3, N_t\}$. 
\yf{HN}{The link between the interaction names and the components is not clear.}
%
A new task generated by \textit{Task generator} needs two workers to be done. New task is delivered through the port \textit{deliver} to two free workers. Delivering a task by \textit{Task generator} is modeled by a move from \textit{ready} to \textit{delivered} location. As soon as each worker receives a task through port \textit{exec}, it moves to the \textit{done} location and increments the value of variable $x$. Moving back from \textit{done} to \textit{free} depends on the value of $x$ such that if the value of $x$ is lesser than or equal to ten, by execution of singleton interaction labeled by port \textit{finish} moves from \textit{done} to \textit{free}, otherwise by another singleton interaction labeled by port \textit{maintenance} moves from \textit{done} to \textit{free} and resets $x$. Generating a new task by \textit{Task generator} is modeled by a transition from \textit{delivered} to \textit{ready} labeled by the port $N_t$.\\
Let us consider $\left(q_1,q_2,q_3,q_4\right)$ as state of the system in which $q_1,q_2,q_3,q_4$ represent the states of  \textit{Worker1}, \textit{Worker2},  \textit{Worker3}, \textit{Task generator} respectively. When all states of the components are defined we have a global state of the system. whenever one or more components is busy with internal computation (denoted by the symbol $\perp$ ), global state of the system is not defined and system's state is partially known. In the sequential execution manner, no interaction is possible when some component is performing a computation, \ie no parallelism is possible.
%
The following trace is a sample execution which points out the fact that in sequential execution where there is only one thread of execution, global state is always available.\\
{\footnotesize $\left(free,free,free,ready\right)\cdot E_{12}\cdot\left(done,done,free,delivered\right)\cdot N_t\cdot\left(done,done,free,ready\right)$}\\
A runtime monitor ~\cite{FalconeJNBB11} consumes global states after interactions to check the system behavior w.r.t the given property.\\
Whereas the principle of concurrent execution is that controller can execute an interaction even in the absence of global state of the system. For instance execution of interaction $E_{12}$ from the initial state $\left(free,free,free,ready\right)$ changes the global state to a partial state which is $\left(\perp,\perp,free,\perp\right)$ then from a partial state, controller has two choices, either waiting for busy component to finish their computation (by $\beta$ transitions) or executing a new possible interaction. The following trace of execution shows that at the time \textit{worker1} and \textit{worker2} are busy, interaction $N_t$ can be fired.\\
{\footnotesize $\left(free,free,free,ready\right)\cdot E_{12}\cdot\left(\perp,\perp,free,\perp\right)\cdot\beta_4\cdot\left(\perp,\perp,free,deliver\right)\cdot N_t\cdot\left(\perp,\perp,free,\perp\right)$}\\
Not having enough information in partial states is the main problem of a runtime monitor. In this paper we introduce a method to reconstruct global states from the partial states of the system such that at a same time we have benefited form parallel execution and runtime monitoring.



%\end{example}
\input{example_global}

==> result_old.tex <==

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
System                                                              & \multicolumn{2}{c|}{no-monitor}                   & \multicolumn{6}{c|}{with monitor}                                                      \\ \hline
\multirow{5}{*}{Temperature Control}                                & time (s)                & steps                   & \multicolumn{2}{c|}{specification}       & steps   & events & time (s) & overhead (\%) \\ \cline{2-9} 
                                                                    & \multirow{4}{*}{146.98} & \multirow{4}{*}{69,753} & Single command             & $\varphi_1$ & 69,785  & 31     & 148.62   & 1.12          \\ \cline{4-9} 
                                                                    &                         &                         & Ordering                   & $\varphi_2$ & 73,352  & 3,589  & 151.05   & 2.76          \\ \cline{4-9} 
                                                                    &                         &                         & Rod resting                & $\varphi_3$ & 73,805  & 4,051  & 157.33   & 7.04          \\ \cline{4-9} 
                                                                    &                         &                         & Availability               & $\varphi_4$ & 76,951  & 7,198  & 158.11   & 7.49          \\ \hline
Readers-Writer                                                      & 61.54                   & 120,000                 & Data freshness             & $\varphi_5$ & 200,000 & 40,000 & 62.144   & 0.98          \\ \hline
\begin{tabular}[c]{@{}c@{}}Readers-Writer\\ (3 Writer)\end{tabular} &18.98                      &40,000                         & Complex execution ordering & $\varphi_7$ & 170,000 & 40,000 & 23.27   & 22.55          \\ \hline
\multirow{2}{*}{Demosaicing}                                        & \multirow{2}{*}{65.98}  & \multirow{2}{*}{840}    & \multirow{2}{*}{Complete process} & $\varphi_8$ & 1,520   & 439    & 66.28    & 0.45          \\ \cline{5-9} 
                                                                    &                         &                         &                                   & $\varphi_9$ &         &        &          &         \\ \hline
\end{tabular}
\caption{Results of monitoring the requirements} 
\label{Table:result1}
\end{table}


==> rgt_table_old.tex <==
\begin{table}
\centering
\caption{Values of function $\RGT$ for a sample input} 
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|}
$\quad$Step$\quad$ & $\quad\quad\quad$\begin{tabular}[c]{@{}c@{}} Input trace in partial semantics \\$\sigma$\end{tabular}$\quad\quad\quad$ & $\quad\quad\quad\quad$\begin{tabular}[c]{@{}c@{}} Intermediate step \\$\Acc(\sigma)$\end{tabular}$\quad\quad\quad\quad$ & $\quad$\begin{tabular}[c]{@{}c@{}} Output trace in global semantics \\$\RGT(\sigma)$ \end{tabular}$\quad$ \\ 
%\rowcolor[HTML]{EFEFEF} 
0 & $(\free,\free,\free,\ready)$ & $(\free,\free,\free,\ready)$ & $(\free,\free,\free,\ready)$ \\ 
1 &\begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}\cdot$\\$(\perp,\perp,\free,\perp)$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}\cdot$\\$(\perp,\perp,\free,\perp)$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}$\end{tabular} \\ 
%\rowcolor[HTML]{EFEFEF} 
2 & \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}\cdot$\\$(\perp,\perp,\free,\perp)\cdot\beta_4\cdot$\\$(\perp,\perp,\free,\delivered)$\end{tabular}  & \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}\cdot$\\$(\perp,\perp,\free,\delivered)$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}$\end{tabular} \\ 
3 & \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}\cdot$\\$(\perp,\perp,\free,\perp)\cdot\beta_4\cdot$\\$(\perp,\perp,\free,\delivered)\cdot n_t\cdot$\\$(\perp,\perp,\free,\perp)$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}\cdot$\\$(\perp,\perp,\free,\delivered)\cdot n_t\cdot$\\$(\perp,\perp,\free,\perp)$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}$\end{tabular} \\ 
%\rowcolor[HTML]{EFEFEF} 
4 & \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}\cdot$\\$(\perp,\perp,\free,\perp)\cdot\beta_4\cdot$\\$(\perp,\perp,\free,\delivered)\cdot n_t\cdot$\\$(\perp,\perp,\free,\perp)\cdot\beta_2\cdot$\\$(\perp,\done,\free,\perp)$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}\cdot$\\$(\perp,\done,\free,\delivered)\cdot n_t\cdot$\\$(\perp,\done,\free,\perp)$\end{tabular} &  \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}$\end{tabular}\\ 
5 & \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}\cdot$\\$(\perp,\perp,\free,\perp)\cdot\beta_4\cdot$\\$(\perp,\perp,\free,\delivered)\cdot n_t\cdot$\\$(\perp,\perp,\free,\perp)\cdot\beta_2\cdot$\\$(\perp,\done,\free,\perp)\cdot\beta_1\cdot$\\$(\done,\done,\free,\perp)$\end{tabular}& \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}\cdot$\\ $(\done,\done,\free,\delivered)\cdot n_t\cdot$\\$(\done,\done,\free,\perp)$\end{tabular} & \begin{tabular}[c]{@{}c@{}}$(\free,\free,\free,\ready)\cdot\ex_{12}\cdot$\\ $(\done,\done,\free,\delivered)\cdot n_t$\end{tabular} \\

\end{tabular}
}
\label{Table:RGT}
\end{table}



==> tempcontrol.tex <==

\subsection{Temperature control system}

\paragraph{Temperature control system.} The system controls the coolant temperature in a reactor tank by moving two independent control rods. The goal is to maintain the coolant between the temperatures $\theta_m$ and $\theta_M$. When the temperature reaches its maximum value $\theta_M$, the tank must be refrigerated with one of the rods. The temperature rises at rate $v_r$ and decreases at rate $v_d$. A rod can be moved again only if $T$ time units have elapsed since the end of its previous movement. If the temperature of the coolant cannot decrease because there is no available rod, a complete shutdown is required.
A BIP model of the Temperature Control System is provided. This model is decomposed into several atomic components: a controller, two components Rod1, Rod2 modeling the rods, one reactor, one temperature component to model the reactor's temperature, two components to model the positions of two rods, two components modeling the commands corresponding to the controller commands for each rod and one monitor component to indicate the system's variables and states. We take $\theta_m = 100$, $\theta_M= 1000$ , $T = 3600$ seconds, and we assume that $v_r=1^\circ/s$  and $v_d=2^\circ/s$. For space reasons, we present a simplified model in Fig. ~\ref{fig:TC} consisting of the controller and two rods components. The components Rod1 and Rod2 are identical, up to the renaming of locations and ports. Each one has two control locations and four transitions: two loop transitions labeled by tick and two transitions synchronized with transitions of the controller. We consider the following properties: (see Fig.~\ref{fig:automata TC})
\paragraph{Single command.}
Commands for moving down can not be sent to more than one rod at a time. This requirement is formalized as $\varphi_1$.\\
 $e_1 : Controller.rod1==down$\\ $e_2 : Controller.rod2==down$\\
\textit{Ordering.}
The rods are initialized at \textit{ready} position. Each time a down command is received, the corresponding rod moves to the \textit{down} position. As soon as the temperature of coolant reaches the desired set point, rod moves to \textit{rest} position. And after $T$ time units it moves back to \textit{ready} position. This order has to be followed by each rod's position. This requirement is formalized as $\varphi_2$.\\
$e_1 : Rod1.position==ready$\\ $e_2 : Rod1.position==down$\\$e_3 : Rod1.position==rest$\\
\textit{Rod resting.}
Rods need to be commanded down one after another i.e., no rod moves to a down position if it was the last one to be there. This requirement is formalized as $\varphi_3$.\\
$e_1 : Rod1.command==down$\\ $e_2 : Rod2.command==down$\\
\textit{Availability.}
At least one rod is in ready position. This requirement is formalized as $\varphi_4$.\\
$e_1 : Monitor.rod1==ready$\\ $e_2 : Monitor.rod2==ready$\\

\begin{figure}[h]
\centering
\scalebox{.6} {
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm, semithick]
  \tikzstyle{every state}=[fill=none,draw=black,text=black]
 
  \node[state] (A)  {$l_1$};
  \node[state] (B) [below of=A,node distance=2cm] {$l_2$};
  \node[state] (C) [right of=A,node distance=5cm] {$l_5$};
  \node[state] (D) [below of=C,node distance=2cm] {$l_6$}; 
  \node[state] (E) [right of=C,node distance=5.5cm] {$l_3$};
  \node[state] (F) [below of=E,node distance=2cm] {$l_4$}; 
  
  \path (A) edge [loop above]  node [label={$t_1=t_1+1$}]{$tick_1$} ();
  \path (B) edge [loop below]  node {$tick_1$} ();
  \path (A) edge [bend right]  node [left,label={$t_1\geq3600\qquad$}]{$cool_1$} (B);
  \path (B) edge [bend right]  node [right,label={$\quad t_1=0$}]{$rest_1$} (A);
  
  
  
  \path (C) edge [loop above]  node [label={$\theta<1000$ , $\theta=\theta+1$}]{$tick$} ();
  \path (D) edge [loop below]  node  {$tick$} ();
  \node [below of=D,node distance=1.6cm]  {$\theta>100$ , $\theta=\theta-2$};
  
  \path (C) edge [bend right]  node [left,label={$\theta==1000\qquad\quad $}]{$cool$} (D);
  \path (D) edge [bend right]  node [right,label={$\qquad \theta==100$}]{$heat$} (C);
  
  
  \path (E) edge [loop above]  node [label={$t_2=t_2+1$}]{$tick_2$} ();
  \path (F) edge [loop below]  node {$tick_2$} ();
  \path (E) edge [bend right]  node [left,label={$t_2\geq3600\qquad$}]{$cool_2$} (F);
  \path (F) edge [bend right]  node [right,label={$\quad t_2=0$}]{$rest_2$} (E);
  
  \filldraw[fill=none,draw=black](-2.5,-4)--(-2.5,2)--(2,2)--(2,-4)--(-2.5,-4)--cycle;
  \fill (-1.7,2) circle (0.1cm);\node at (-2.2,2.2){$rest_1$};
  \fill (1.2,2) circle (0.1cm);\node at (0.7,2.2){$cool_1$};
  \fill (-1.7,-4) circle (0.1cm);\node at (-2.2,-4.2){$tick_1$};
  \node at (0,-4.3) {\textbf{Rod1}};
  \filldraw[fill=none,draw=black,xshift=5cm](-2.5,-4)--(-2.5,2)--(2.4,2)--(2.4,-4)--(-2.5,-4)--cycle;
  \fill (3.3,2) circle (0.1cm);\node at (2.8,2.2){$cool$};
  \fill (6.5,2) circle (0.1cm);\node at (6,2.2){$heat$};
  \fill (3.3,-4) circle (0.1cm);\node at (2.8,-4.2){$tick$};
  \node at (5,-4.3) {\textbf{Controller}};
  \filldraw[fill=none,draw=black,xshift=10.5cm](-2.5,-4)--(-2.5,2)--(2,2)--(2,-4)--(-2.5,-4)--cycle;
  \fill (8.8,2) circle (0.1cm);\node at (8.2,2.2){$rest_2$};
  \fill (11.7,2) circle (0.1cm);\node at (11.2,2.2){$cool_2$};
  \fill (8.8,-4) circle (0.1cm);\node at (8.2,-4.2){$tick_2$};
  \node at (10.5,-4.3) {\textbf{Rod2}};
  
  \draw[-] (-1.7,-4)--(-1.2,-5)--(8.3,-5)--(8.8,-4); 
  \draw[-] (3.3,-4)--(3.3,-5.02); 
  \draw[-] (-1.7,2)--(-1.2,2.8)--(8.3,2.8)--(8.8,2);
  \draw[-] (6.5,2)--(6.5,2.82);
  \draw[-] (1.2,2)--(1.7,3.1)--(11.2,3.1)--(11.7,2);
  \draw[-] (3.3,2)--(3.3,3.13);

            
\end{tikzpicture}
}
\caption{Temperature control system}
\label{fig:TC} 
\end{figure}





\begin{figure}[h]
    \centering
    \begin{minipage}{.3\textwidth}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \scalebox{.5} {\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm, semithick,baseline=-0.3cm]
  \node[state,initial] (A)  {$S_1$};
  \path (A) edge [loop right]    node {$\neg e_1 \vee \neg e_2 $} ();              
  \addvmargin{3mm}
\end{tikzpicture}}
        \caption{$\varphi_1$}
        \label{fig:phi1}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{\textwidth}
        \centering
    \scalebox{.5} {
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm, semithick,baseline=-0.3cm]

  \node[state,initial] (A)  {$S_1$};
  \node[state]         (B) [above right of=A,node distance=1.6cm] {$S_2$};
  \node[state]         (C) [below right of=A,node distance=1.6cm] {$S_3$};
  \path (A) edge [bend left]               node {$e_1$} (B); 
  \path (B) edge [bend left]               node {$e_2$} (C);
  \path (C) edge [bend left]               node {$e_3$} (A);
  \addvmargin{2mm}         
\end{tikzpicture}
}
        \caption{$\varphi_2$}
        \label{fig:phi2}
    \end{subfigure}
    \end{minipage}
    \begin{minipage}{.3\textwidth}
    \hfill
            \begin{subfigure}[b]{\textwidth}
        \centering
\scalebox{.5} {
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm, semithick,baseline=-0.3cm]
  \node[state,initial]         (A)              {$S_1$};
  \node[state]         (D) [right of=A,node distance=3cm] {$S_5$};
  \node[state]         (F) [right of=D,node distance=2.8cm] {$S_3$};
  \node[state]         (B) [above right of=D,node distance=2cm] {$S_2$};
  \node[state]         (C) [below right of=D,node distance=2cm] {$S_4$};
  \path (A) edge [loop above]      node {$\neg e_1 \wedge \neg e_2$} ();
  \path (A) edge [bend left]        node {$e_1$} (B);
  \path (B) edge [loop above]       node {$e_1$} ();
  \path (A) edge [bend right]       node {$e_2$} (C);
  \path (D) edge                    node {$e_1$} (B);
  \path (B) edge                    node {$\neg e_1$} (F);
  \path (F) edge                    node {$e_2$} (C);
  \path (C) edge                    node {$\neg e_2$} (D);
  \path (F) edge [loop right]       node {$\neg e_1 \wedge \neg e_2$} ();
  \path (C) edge [loop below]       node {$e_2$} ();
  \path (D) edge [loop left]        node {$\neg e_1 \wedge \neg e_2$} ();
  \addvmargin{2mm}              
\end{tikzpicture}
}
        \caption{$\varphi_3$}
        \label{fig:phi3}
    \end{subfigure}
    \end{minipage}
    \begin{minipage}{.3\textwidth}
    \begin{subfigure}[b]{\textwidth}
        \centering
\scalebox{.5} {
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm, semithick,baseline=-0.3cm]
  \node[state,initial]         (A)              {$S_1$};
  \node[state]         (D) [right of=A,node distance=3cm] {$S_5$};
  \node[state]         (F) [right of=D,node distance=2.8cm] {$S_3$};
  \node[state]         (B) [above right of=D,node distance=2cm] {$S_2$};
  \node[state]         (C) [below right of=D,node distance=2cm] {$S_4$};
  \path (A) edge [loop above]      node {$\neg e_1 \wedge \neg e_2$} ();
  \path (A) edge [bend left]        node {$e_1$} (B);
  \path (B) edge [loop above]       node {$e_1$} ();
  \path (A) edge [bend right]       node {$e_2$} (C);
  \path (D) edge                    node {$e_1$} (B);
  \path (B) edge                    node {$\neg e_1$} (F);
  \path (F) edge                    node {$e_2$} (C);
  \path (C) edge                    node {$\neg e_2$} (D);
  \path (F) edge [loop right]       node {$\neg e_1 \wedge \neg e_2$} ();
  \path (C) edge [loop below]       node {$e_2$} ();
  \path (D) edge [loop left]        node {$\neg e_1 \wedge \neg e_2$} ();
  \addvmargin{2mm}              
\end{tikzpicture}
}
        \caption{$\varphi_4$}
        \label{fig:phi4}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{\textwidth}
        \centering
\scalebox{.5} {
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.8cm, semithick,baseline=-0.3cm]
  \node[state,initial]         (D)  {$S_1$};
  \node[state]         (E) [right of=D,node distance=5cm] {$S_2$};
  \path (D) edge node{$(e_1\wedge\neg e_2)\vee (\neg e_1\wedge e_2)$} (E);
  \path (E) edge [bend left]  node {$e_1 \wedge e_2$} (D);
  \path (E) edge [loop above] node {$(e_1\wedge\neg e_2)\vee(\neg e_1 \wedge e_2)$} ();
  \path (D) edge [loop above] node {$e_1 \wedge e_2$} ();
   \addvmargin{2mm}          
\end{tikzpicture}
}
        \caption{$\varphi_5$}
        \label{fig:phi5}
    \end{subfigure}
    \end{minipage}
    \caption{Automata of properties of temperature control system}
    \label{fig:automata TC}
\end{figure}





